A type A structure in Khovanov Homology

Inspired by bordered Floer homology, we describe a type A structure on a Khovanov homology for a tangle, which complements the type D structure in a previous paper. The type A structure is a differential module over a certain algebra. This can be paired with the type D structure to recover the Khovanov chain complex. The homotopy type of the type A structure is a tangle invariant, and homotopy equivalences of the type A structure result in chain homotopy equivalences on the Khovanov chain complex. We can use this to simplify computations and introduce a modular approach to the computation of Khovanov homologies. This approach adds to the literature even in the case of a connect sum, where the techniques here will allow an exact computation of Khovanov homology from the structures for two tangles coming from the summands. Several examples are included, showing in particular how we can compute the correct torsion summands for the Khovanov homology of the connect sum. A lengthy appendix is devoted to establishing the theory of these structures over a characterstic zero ring.

==> cleaverSignsMatchingSummaryA.June5.tex <==
\section{The algebra from cleaved links}\label{sec:algebra}

\noindent We summarize the construction of the algebra $\mathcal{B}\Gamma_{n}$ from \cite{typeD}. 

\subsection{Cleaved planar links}

\noindent Let $P_{n}$ be the set of points $p_{1}=(0,1),\ldots, p_{2n}=(0,2n)$ on the $y$-axis of $\R^{2}$, ordered by the second coordinate. We denote the closed half-plane $(-\infty,0] \times \R \subset \R^{2}$ by $\leftHalf$ while  $\rightHalf = [0,\infty) \times \R$. 

\begin{defn}
A {\em $n$-cleaved link} $L$ is an embedding of circles in $\R^{2}$ such that 
\begin{enumerate}
\item the circles of $L$ are disjoint and transverse to the $y$-axis,
\item each point in $P_{n}$ is on a circle in $L$,
\item each circle in $L$ contains at least two points in $P_{n}$
\end{enumerate}
The set of circle components of $L$ will be denoted $\circles{L}$.
\end{defn}

\noindent We take two $n$-cleaved links to be equivalent if they are related by an isotopy of $\R^{2}$ which pointwise fixes the $y$-axis, and by reversing the orientation on each circle. We will denote the equivalence classes by $\cleave{n}$

\begin{defn}
The {\em constituents} of an $n$-cleaved link $L$ are the planar matchings:
\begin{equation}
\lefty{L} = \leftHalf \cap L  \hspace{1in}
\righty{L} = \rightHalf \cap L 
\end{equation}
\end{defn}

\begin{defn}
A {\em bridge} for a cleaved link $L$ is an embedding $\gamma : [0,1] \rightarrow \R^{2}\backslash \big(\{0\}\times \R\big)$ such that 
\begin{enumerate}
\item $\gamma(0)$ and  $\gamma(1)$ are on {\em distinct} of $\lefty{L}$ or $\righty{L}$
\item the image under $\gamma$ of $(0,1)$ is disjoint from $L$ 
\end{enumerate} 
\end{defn}

\noindent By definition, a bridge $\gamma$ has image in either $\rightHalf$ or $\leftHalf$. We call this half plane the {\em location} of the bridge. Bridges are also considered up to isotopy fixing the $y$-axis. 

\begin{defn}
The equivalence classes of bridges for a cleaved link $L$ will be denoted $\bridges{L}$. $\bridges{L} = \leftBridges{L} \cup \rightBridges{L}$ where $\leftBridges{L}$ consists of those equivalence classes in $\leftHalf$ and $\rightBridges{L}$ consists of those classes in $\rightHalf$.
\end{defn}

\noindent For each class of bridges $\gamma \in \bridges{L}$ we can construct a new cleaved planar link. 

\begin{defn}
Let $L$ be an equivalence class of cleaved links and let $\gamma \in \bridges{L}$. $L_{\gamma}$ is the equivalence class of cleaved links found by surgery along $\gamma$. 
\end{defn}

\noindent $L_{\gamma}$ has a special bridge $\gamma^{\dagger}$ introduced by the surgery. More specifically, there is a neighborhood of $\gamma$ homeomorphic to $[-1,1] \times [-1,1]$ which intersects $L$ along $\{\pm 1\}\times[-1,1]$, and for which $\gamma$ is $[-1,1] \times \{0\}$ (i.e. the core). $L_{\gamma}$ results from removing these two arcs from $L$ and replacing them with $[-1,1] \times \{\pm 1\}$. $\gamma^{\dagger}$ is then the bridge for $L_{\gamma}$ defined by the arc $\{0\} \times [-1,1]$.  

\begin{defn}
\begin{enumerate}
\item The support of $\gamma \in \bridges{L}$ is the set of {\em three} circles in $L$ and $L_{\gamma}$ which contain the feet of $\gamma$ and $\gamma^{\dagger}$
\item $\merge{L}$ is the subset of $\gamma \in \bridges{L}$ where surgery on $\gamma$ merges two circles $\{\startCircle{\gamma}, \terminalCircle{\gamma}\}$. In this case, $C_{\gamma}$ is the circle in $\circles{L_{\gamma}}$ which contains both feet of $\gamma^{\dagger}$.
\item $\fission{L}$ is the subset of $\gamma \in \bridges{L}$ where surgery on $\gamma$ divides a circle $C$ of $L$. In this case, $C^{a}_{\gamma}$ and $C^{b}_{\gamma}$ are the circles in $\circles{L_{\gamma}}$ which contain the feet of $\gamma^{\dagger}$.   
\end{enumerate}
\end{defn}

\begin{prop}
Given any bridge $\gamma$ for $L$, $\bridges{L}\backslash\{\gamma\}$ can be decomposed as a union $B_{\pitchfork}(L,\gamma) \cup B_{|\,|}(L,\gamma)$, where
\begin{enumerate}
\item $B_{|\,|}(L,\gamma)$ consists of the classes of bridges containing a representative which does not intersect $\gamma$,
\item $B_{\pitchfork}(T,\gamma)$ consists of the classes of bridges all of whose representatives intersect $\gamma$
\end{enumerate}  
\end{prop}

\noindent Note that if $\eta \in B_{|\,|}(L,\gamma)$ then $\gamma \in B_{|\,|}(L,\eta)$. There is an identification of $B_{|\,|}(L_{\gamma}, \gamma^{\dagger})$ with $B_{|\,|}(L,\gamma)$. 


\noindent A {\em decoration} for an $n$-cleaved link $L$ is a map $\sigma\!: \circles{L} \lra \{+,-\}$. 

\begin{defn}
$\cleaved{n}$ is the set of decorated, $n$-cleaved links:
\begin{equation}
\cleaved{n}= \big\{\,(L,\sigma)\,\big|\,L\in \cleave{n}, \sigma\mathrm{\ is\ a\ decoration\ for\ }L\big\}
\end{equation} 
\end{defn}

\noindent We will often restrict a decoration $\sigma$ of $L$ to give decorations on the arcs of its constituents $\lefty{L}$ and  $\righty{L}$. In addition, we will need to following statistic for a decorated, cleaved link:
\begin{equation}
\iota(L,\sigma) = \#\big\{C \in \circles{L} \big| \sigma(C) = +\big\} - \#\big\{C \in \circles{L} \big| \sigma(C) = -\big\}
\end{equation}


\subsection{The algebra $\mathcal{B}\Gamma_{n}$}

\noindent We will describe $\mathcal{B}\Gamma_{n}$ by generators and relations. First, there is an idempotent for each decorated, cleaved link in $\cleaved{n}$. We will denote the idempotent corresponding to $(L,\sigma)$ by $I_{(L,\sigma)}$. The idempotents will be orthogonal to each other. 

\begin{defn}
$\mathcal{I}_{n}$ is the sub-algebra generated by the idempotents $I_{(L,\sigma)}$.
\end{defn}

\noindent For each $(L,\sigma) \in \cleaved{n}$ we specify certain elements in $I_{(L,\sigma)}\mathcal{B}\Gamma_{n}$. $\mathcal{B}\Gamma_{n}$ will be freely generated by the idempotents and these elements, subject to the relations described below.
\begin{enumerate}
\item For each circle $C \in \circles{L}$ with $\sigma(C) = +$ there are two elements $\righty{e_{C}}$ and $\lefty{e_{C}}$ in 
$I_{(L,\sigma)}\mathcal{B}\Gamma_{n}$. Furthermore, $\righty{e_{C}}I_{(L,s_{C})} = \righty{e_{C}}$ for the decoration with $s_{C}(C) = -$ and $s_{C}(D) = s(D)$ for each $D \in \circles{L}\backslash\{C\}$, while $\righty{e_{C}}I_{(L',s')} = 0$ for every other idempotent. The same relations hold for $\lefty{e_{C}}$. These types of elements are called {\em decoration elements}, while the $C$ above is called the {\em support} of the element.
\item Let $\gamma \in \bridges{L}$, then there is a {\em bridge element} $e_{(\gamma; \sigma , \sigma_{\gamma})}$ with $I_{(L,\sigma)}e_{(\gamma; \sigma , \sigma_{\gamma})} = e_{(\gamma; \sigma , \sigma_{\gamma})}I_{(L_{\gamma},\sigma_{\gamma})} = e_{(\gamma; \sigma , \sigma_{\gamma})}$ in each of the following cases, based on the decorations,
\begin{enumerate}
\item\label{bridge1} when  $\gamma \in \merge{L}$ and $\sigma$ and $\sigma_{\gamma}$ restrict to the support of $\gamma$ as one of 
$$
\begin{array}{llcl}
\sigma(\startCircle{\gamma})=+ & \sigma(\terminalCircle{\gamma})= + &\hspace{1in} &\sigma_{\gamma}(C_{\gamma})= + \\
\sigma(\startCircle{\gamma})=- & \sigma(\terminalCircle{\gamma})= + &\  &\sigma_{\gamma}(C_{\gamma})= - \\
\sigma(\startCircle{\gamma})=+ & \sigma(\terminalCircle{\gamma})= - &\ &\sigma_{\gamma}(C_{\gamma})= - \\
\end{array}
$$ 
and $s(D)=s_{\gamma}(D)$ on every circle not in the support of $\gamma$;
\item\label{bridge2} when $\gamma \in \fission{L}$, $C \in \circles{L}$ is the circle containing both feet of $\gamma$, and
\begin{enumerate}
\item  $\sigma(C) = +$,  if $\sigma$ and $\sigma_{\gamma}$ restrict to the support of $\gamma$ as either of
$$
\begin{array}{llcl}
\sigma(C)=+ &\hspace{1in} & \sigma_{\gamma}(C^{a}_{\gamma})= + & \sigma_{\gamma}(C^{b}_{\gamma})= - \\
\sigma(C)=+ &\ & \sigma_{\gamma}(C^{a}_{\gamma})= - & \sigma_{\gamma}(C^{b}_{\gamma})= + \\
\end{array}
$$
\item $\sigma(C) = -$, if $\sigma$ and $\sigma_{\gamma}$ restrict to the support of $\gamma$ as 
$$
\begin{array}{llcl}
\sigma(C)=- & \hspace{1in} & \sigma^{-}_{\gamma}(C^{a}_{\gamma})= - & \sigma^{-}_{\gamma}(C^{b}_{\gamma})= - \\
\end{array}
$$
\end{enumerate}
and $s(D)=s_{\gamma}(D)$ on every circle not in the support of $\gamma$.
\end{enumerate}
\end{enumerate}

\noindent In \cite{typeD} we note that with these generators and idempotents
\begin{prop}
$\mathcal{B}\bridgeGraph{n}$ is finite dimensional
\end{prop}

\noindent Furthermore, $\mathcal{B}\bridgeGraph{n}$ can be given a bigrading, \cite{typeD}. On the generating elements the bigrading is specified by setting
$$
\begin{array}{lcl}
\mathrm{I}_{(L,\sigma)} & \longrightarrow & (0,0)\\
\righty{e_{C}} & \longrightarrow & (0,-1)\\
\lefty{e_{C}} & \longrightarrow & (1,1)\\
\righty{e_{\gamma}} &\longrightarrow & (0,-1/2)\\
\lefty{e_{\gamma}} &\longrightarrow & (1,1/2)\\
\end{array}
$$
\noindent On every other element it is computed by extending the above homomorphically. The first entry of this bigrading will be denoted $\leftnorm{\alpha}$, while the second element will be denoted $q(\alpha)$.\\
\ \\
\noindent We now turn to describing the relations between these generators. Each of the relations is homogeneous with respect to the bigrading. First, there are a number of ``graded commutativity'' relations, based on the first entry in the bigrading:
\begin{equation}
e_{\alpha}e_{\beta'} = (-1)^{\leftnorm{e_{\alpha}}\leftnorm{e_{\beta}}}e_{\beta}e_{\alpha'} 
\end{equation}
This graded commutativity occurs in the following cases, assuming that $I_{(L,\sigma)}e_{\alpha} \neq 0$ and $I_{(L,\sigma)}e_{\beta} \neq 0$, 
\begin{enumerate}
\item If $e_{\alpha}$ and $e_{\beta}$ are decoration elements for distinct circles $C$ and $D$ in $(L,\sigma)$ with $\sigma(C)=\sigma(D)=+$, and $e_{\alpha'}$ is the decoration element for $D$ in $(L,\sigma_{C})$, while $e_{\beta'}$ is the
decoration element for $C$ in $(L,\sigma_{D})$.
\item If $e_{\alpha}=e_{(\gamma,\sigma,\sigma')}$ for a bridge $\gamma$ in $(L,\sigma)$ and $e_{\beta}$ is a decoration element for $C \in \circles{L}$, with $C$  not in the support of $\gamma$, while $e_{\alpha'} = e_{(\gamma,\sigma_{C},\sigma_{C}')}$ and $e_{\beta'}$ is the decoration element for $C$ in $(L_{\gamma},s')$. Due to the disjoint support, there will always be a pair of such elements.
\item If $e_{\alpha}= e_{(\gamma,\sigma,\sigma')}$ and $e_{\beta}=e_{(\eta,\sigma,\sigma'')}$ are bridge elements for distinct bridges $\gamma$ and $\eta$ in $(L,\sigma)$, where, in addition, 1) $\eta \in B_{|\,|}(L,\gamma)$, and 2) $\eta$ and $\gamma$ either have disjoint support or at least one is a right bridge edge, and 3) $e_{\beta'}= e_{(\eta,\sigma',\sigma''')}$ and $e_{\alpha'}=e_{(\gamma,\sigma'',\sigma''')}$ for some decoration $\sigma'''$ on $L_{\gamma,\eta}$.
\end{enumerate}

\noindent We note that the type (decoration vs. bridge) and the location are the same for $e_{\alpha}$ and $e_{\alpha'}$ as well as for the pair $e_{\beta}$ and $e_{\beta'}$. In fact, in all these relations elements of the algebra from $\rightHalf$ will act like even elements for the $\Z/2\Z$-grading from $\leftnorm{\alpha}$, while elements from $\leftHalf$ act like {\em odd} elements.\\
\ \\
\noindent {\bf Other bridge relations:} Suppose $\gamma \in \leftBridges{L}$ and $\eta \in B_{\pitchfork}(L_{\gamma},\gamma^{\dagger})$, then 
$$
e_{(\gamma,\sigma,\sigma')}e_{(\eta,\sigma',\sigma'')} = 0
$$
whenever $\sigma'$ and $\sigma''$ are compatible decorations.\\
\ \\
\noindent Furthermore, suppose that there is a circle $C \in \circles{L}$ with $\sigma(C)=+$, and there are elements $\righty{e}_{(\gamma,\sigma,\sigma')}$ and $\righty{e}_{(\gamma^{\dagger},\sigma',\sigma_{C})}$ for a bridge $\gamma \in \rightBridges{L}$ then
\begin{equation}\label{rel:special}
\righty{e}_{(\gamma,\sigma,\sigma')}\righty{e}_{(\gamma^{\dagger},\sigma',\sigma_{C})} = \righty{e_{C}}
\end{equation}
Such a circle $C$ is unique for the choice of $\gamma$ and $\sigma'$ and is called the {\em active circle} for $\gamma$.  \\
\ \\
\noindent{\bf Relations for decoration edges:} When the support of $e_{C}$ is not disjoint from that of $\righty{e}_{(\gamma,\sigma,\sigma_{\gamma})}$ the relations are different depending upon the location of $e_{C}$.

\begin{enumerate}
\item {\bf The relations for $\righty{e_{C}}$:} Suppose that $\gamma \in \merge{L}$ merges $C_{1}$ and $C_{2}$ to get $C \in \circles{L_{\gamma}}$, and $\sigma(C_{1}) = \sigma(C_{2}) = +$, then
\begin{equation}
\righty{e_{C_{1}}}m_{(\gamma,\sigma_{C_{1}},\sigma_{C})} = \righty{e_{C_{2}}}m_{(\gamma,\sigma_{C_{2}},\sigma_{C})} = m_{(\gamma,\sigma,\sigma_{\gamma})} \righty{e_{C}}
\end{equation}
Note that if $\sigma(C_{i}) = -$ for either $i=1$ or $2$, then there is no relation imposed. \\
\ \\
Dually, if surgery on $\gamma \in \fission{L}$ divides circle $C \in \circles{L}$ into $C_{1}$ and $C_{2}$ in $\circles{L_{\gamma}}$, and $\sigma$ assigns $+$ to $C$, then 
\begin{equation}
\righty{e_{C}}f_{(\gamma,\sigma_{C},\sigma_{C,\gamma})} =  f_{(\gamma,\sigma,\sigma^{1}_{\gamma})}\righty{e_{C_{1}}} = f_{(\gamma,\sigma,\sigma^{2}_{\gamma})} \righty{e_{C_{2}}}
\end{equation}
where $\sigma^{i}_{\gamma}$ assigns $+$ to $C_{i}$ and $-$ to $C_{3-i}$. 

\item {\bf The relations for $\lefty{e_{C}}$:} Suppose that $\gamma \in \rightMerge{L}$ merges $C_{1}$ and $C_{2}$ to get $C \in \circles{L_{\gamma}}$, and $\sigma(C_{1}) = \sigma(C_{2}) = +$, then:
\begin{equation}\label{rel:lefty1}
\lefty{e_{C_{1}}}m_{(\gamma,\sigma_{C_{1}},\sigma_{C})} + \lefty{e_{C_{2}}}m_{(\gamma,\sigma_{C_{2}},\sigma_{C})} - m_{(\gamma,\sigma,\sigma_{\gamma})} \lefty{e_{C}} = 0
\end{equation}
and when $\sigma(C) = +$ and $\gamma \in \rightFission{L}$ divides $C$ into $C_{1}$ and $C_{2}$
\begin{equation}\label{rel:lefty2}
\lefty{e_{C}}f_{(\gamma,\sigma_{C},\sigma_{C,\gamma})} +  f_{(\gamma,\sigma,\sigma^{1}_{\gamma})}\lefty{e_{C_{1}}} - f_{(\gamma,\sigma,\sigma^{2}_{\gamma})} \lefty{e_{C_{2}}} = 0
\end{equation}
whereas if $\gamma \in \leftMerge{L}$ merges $C_{1}$ and $C_{2}$ to get $C \in \circles{L_{\gamma}}$, and $\sigma(C_{1}) = \sigma(C_{2}) = +$, then:
\begin{equation}\label{rel:lefty3}
\lefty{e_{C_{1}}}m_{(\gamma,\sigma_{C_{1}},\sigma_{C})} + \lefty{e_{C_{2}}}m_{(\gamma,\sigma_{C_{2}},\sigma_{C})} + m_{(\gamma,\sigma,\sigma_{\gamma})} \lefty{e_{C}} = 0
\end{equation}
and when $\sigma(C) = +$ and $\gamma \in \leftFission{L}$ divides $C$ into $C_{1}$ and $C_{2}$
\begin{equation}\label{rel:lefty4}
\lefty{e_{C}}f_{(\gamma,\sigma_{C},\sigma_{C,\gamma})} +  f_{(\gamma,\sigma,\sigma^{1}_{\gamma})}\lefty{e_{C_{1}}} + f_{(\gamma,\sigma,\sigma^{2}_{\gamma})} \lefty{e_{C_{2}}} = 0
\end{equation}
\end{enumerate}





\subsection{A differential on $\mathcal{B}\bridgeGraph{n}$}

\noindent Surgery along a bridge $\gamma \in \leftBridges{L}$ followed surgery on $\gamma^{\dagger}$ {\em does not} correspond to a relation (compare relation \ref{rel:special}). Instead these products occur in a differential on $\mathcal{B}\bridgeGraph{n}$.

\begin{prop}\cite{typeD}
Let $(L,\sigma) \in \cleaved{n}$ such that there is a circle $C \in \circles{L}$ with $\sigma(C) = +$. Let $\lefty{e_{C}}$ be
the decoration element corresponding to $C$. Let
\begin{equation}\label{eq:dga}
d_{\Gamma_{n}}(\lefty{e_{C}}) = -\sum e_{(\gamma,\sigma,\sigma_{\gamma})}e_{(\gamma^{\dagger},\sigma_{\gamma},\sigma_{C})}
\end{equation}
where the sum is over all $\gamma \in \leftBridges{L}$ with $C$ as active circle, and all decorations $\sigma_{\gamma}$ which define
compatible elements. Let $d_{\Gamma_{n}}(e) = 0$ for every other generator $e$ (including idempotents). Then $d_{\Gamma_{n}}$ can be extended to a $(1,0)$ differential on bigraded algebra $\mathcal{B}\bridgeGraph{n}$ which satisfies the following Leibniz identity:
\begin{equation}\label{eqn:Leibniz}
d_{\Gamma_{n}}(\alpha\beta) = (-1)^{\leftnorm{\beta}}(d_{\Gamma_{n}}(\alpha)\big)\beta + \alpha\big(d_{\Gamma_{n}}(\beta)\big)
\end{equation}
\end{prop}

\noindent $(\mathcal{B}\bridgeGraph{n}, d_{\Gamma_{n}})$ denotes this differential, bigraded $\Z$-algebra.  \\
\ \\
\subsection{Example:} $(\mathcal{B}\bridgeGraph{1}, d_{\Gamma_{1}})$: $P_{1}$ consists of two points, and there is only one planar matching in $\leftHalf$ and $\rightHalf$. Consequently, the only $1$-cleaved link is a circle intersecting the $y$-axis in two points. Thus, there are two vertices in $\bridgeGraph{1}$: when this circle is decorated with a $+$ and when it is decorated with a $-$. We will call these $C^{\pm}$. There are no bridges in either $\leftHalf$ or $\rightHalf$, so the only edges are $\lefty{e}_{C}: C^{+} \longrightarrow C^{-}$ and  $\righty{e}_{C}: C^{+} \longrightarrow C^{-}$. Thus $\bridgeGraph{1}$ looks like  

\begin{center}
\includegraphics[scale=0.5]{./images/bridgeGraph1}
\end{center}

\noindent Thus, $\mathcal{B}\bridgeGraph{1}$ consists of four elements $I_{C^{+}}, I_{C^{-}}$ in grading $(0,0)$, $\lefty{e}_{C}$ in grading $(1,1)$, and $\righty{e}_{C}$ in grading $(0,-\frac{1}{2})$. The product of any two of these is trivial except for the actions of the idempotents: $I_{C^{+}}\lefty{e}_{C} = \lefty{e}_{C} = \lefty{e}_{C}I_{C^{-}}$, and similarly for $\righty{e}_{C}$. The differential $d_{\Gamma_{1}} \equiv 0$ since its image is in the set generated by paths of bridge edges.\\
\ \\
\noindent For more detail about $(\mathcal{B}\bridgeGraph{2}, d_{\Gamma_{2}})$ see the examples in section 2 of \cite{typeD}.



